ExposureDiffusion: Learning to Expose for Low-light Image Enhancement

Previous raw image-based low-light image enhancement methods predominantly relied on feed-forward neural networks to learn deterministic mappings from low-light to normally-exposed images. However, they failed to capture critical distribution information, leading to visually undesirable results. This work addresses the issue by seamlessly integrating a diffusion model with a physics-based exposure model. Different from a vanilla diffusion model that has to perform Gaussian denoising, with the injected physics-based exposure model, our restoration process can directly start from a noisy image instead of pure noise. As such, our method obtains significantly improved performance and reduced inference time compared with vanilla diffusion models. To make full use of the advantages of different intermediate steps, we further propose an adaptive residual layer that effectively screens out the side-effect in the iterative refinement when the intermediate results have been already well-exposed. The proposed framework can work with both real-paired datasets, SOTA noise models, and different backbone networks. Note that, the proposed framework is compatible with real-paired datasets, real/synthetic noise models, and different backbone networks. We evaluate the proposed method on various public benchmarks, achieving promising results with consistent improvements using different exposure models and backbones. Besides, the proposed method achieves better generalization capacity for unseen amplifying ratios and better performance than a larger feedforward neural model when few parameters are adopted.

==> content/tables.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lccc}
    \hline & $\times 100$ & $\times 250$ & $\times 300$ \\
    Model & PSNR / SSIM  & PSNR / SSIM & PSNR / SSIM \\
    \hline BM3D & $32.92 / 0.758$ & $29.56 / 0.686$ & $28.88 / 0.674$ \\
    \hline A-BM3D & $33.79 / 0.743$ & $27.24 / 0.518$ & $26.52 / 0.558$ \\
    \hline \hline Paired real data & $38.60 / 0.912$ & $37.08 / 0.886$ & $36.29 / 0.874$ \\
    \hline Noise2Noise & $37.42 / 0.853$ & $33.48 / 0.725$ & $32.37 / 0.686$ \\
    \hline \hline$G$ & $36.10 / 0.800$ & $31.87 / 0.640$ & $30.99 / 0.624$ \\
    \hline$G+P$ & $37.08 / 0.839$ & $32.85 / 0.697$ & $31.87 / 0.665$ \\
    \hline$G+P^*$ & $38.31 / 0.884$ & $34.39 / 0.765$ & $33.37 / 0.730$ \\
    \hline$G^*+P^*$ & $39.10 / 0.911$ & $36.46 / 0.869$ & $35.69 / 0.855$ \\
    \hline$G^*+P^*+R$ & $39.23 / 0.912$ & $36.89 / 0.877$ & $36.01 / 0.864$ \\
    \hline$G^*+P^*+R+U$ & $39.27 / 0.914$ & $37.13 / 0.883$ & $36.30 / 0.872$ \\
    \hline \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
\subsection{Results on ELD dataset}
